Scalable K-Medoids via True Error Bound and Familywise Bandits

K-Medoids(KM) is a standard clustering method, used extensively on semi-metric data.Error analyses of KM have traditionally used an in-sample notion of error,which can be far from the true error and suffer from generalization gap. We formalize the true K-Medoid error based on the underlying data distribution.We decompose the true error into fundamental statistical problems of: minimum estimation (ME) and minimum mean estimation (MME). We provide a convergence result for MME. We show $\errMME$ decreases no slower than $\Theta(\frac{1}{n^{\frac{2}{3}}})$, where $n$ is a measure of sample size. Inspired by this bound, we propose a computationally efficient, distributed KM algorithm namely MCPAM. MCPAM has expected runtime $\mathcal{O}(km)$,where $k$ is the number of medoids and $m$ is number of samples. MCPAM provides massive computational savings for a small tradeoff in accuracy. We verify the quality and scaling properties of MCPAM on various datasets. And achieve the hitherto unachieved feat of calculating the KM of 1 billion points on semi-metric spaces.

==> medoid_as_mean_median.tex <==
\chapter{The Medoid as Generalization of Mean and Median}
\label{chapter_medoid_as_generalization_of_mean_and_median}
\ifdraft
TODO: NOTATION IS OUT OF SYNC WITH REST OF PAPER.
\fi
We examine two special cases of the medoid.
When $(\mathcal{M},d) = (\mathbb{R}, \|.\|_2)$ and for any distribution $\mathcal{D}$ we have:
\begin{eqnarray*}
\medoid_2 = \argmin_{x \in \mathbb{R}} \mathbb{E}_Y (Y - x)^2
\end{eqnarray*}
We know from basic probability that the minimizer is the mean and
the minimum $\Ecc_2$ is the variance
\footnote{
The case of squared dissimilarites is briefly considered in the original PAM paper \cite{PAM}.
}.

\ifdraft
TODO: The N-D case for mean.
\fi
When $(\mathcal{M},d) = (\mathbb{R}, \|.\|_1)$ we have:
\begin{eqnarray*}
\medoid_1 = \argmin_{x \in \mathbb{R}} \mathbb{E}_Y |Y - x|
\end{eqnarray*}
Basic probability tells us that the minimizer is the median.
Hence the medoid generalizes both the concepts of mean and median.
We emphasize that in general the medoid is neither the mean nor the median.
For instance, on a space of strings of length $l$ equipped with the Hamming metric
the medoid is well defined, whereas the mean does not exist.
Again, for the subject similarity example (\ifdraft TODO: rewrite this sentence \fi) given in \cite{PAM} neither mean nor
median exist while the medoid does.

\begin{example}
To illustrate the above, consider PAM on iid data $\{X_i\}$, $i \in [1,m]$ 
from a standard normal distribution $\normalDistribution(0,1)$
with the squared Euclidean metric and $k = 1$.
Set $\kTupleSample = \{X_i\}$.
Eccentricity of $x \in \mathbb{R}$ is the second moment of $\normalDistribution(0,1)$ around $x$.
True medoid $\medoid$ is the $x \in \mathbb{R}$ that minimizes this shifted second moment.
$\trueEccSampleMedoid$ is the minimizer over $\{X_i\}$ of this shifted second moment.
Hence the medoid $\medoid$ is nothing but the mean $0$ and the eccentricity of the medoid
is merely the variance $1$.
Set $\SecondarySampleDoubleIndexed = \{X_{j}\}$, $j = [1,m]$.
The sample eccentricity is squared distance to the points in the sample.
The sample medoid is minimizing this over the sample points i.e. merely the sample mean.
For a more general view of the medoid as a generalization of common centrality measures
 (mean and median) refer to appendix 
\ref{chapter_medoid_as_generalization_of_mean_and_median}.
\end{example}


==> pictures/quality_with_avg.tex <==
%\begin{table}[]
\centering
\scalebox{0.7}{
\begin{tabular}{@{}|l|l|l|l|l|l|@{}}
\toprule
\textbf{Dataset} & \textbf{PAM-ARI} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}MCPAM-ARI\\ (mean)\end{tabular}}} & \textbf{DBSCAN-ARI} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}MCPAM \\ rel. err\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}DBSCAN \\ rel. err\end{tabular}}} \\ \midrule
S1 & 0.986 & 0.983 & 0.947 & 0.268 & 3.909 \\ \midrule
S2 & 0.933 & 0.919 & 0.664 & 1.499 & 28.818 \\ \midrule
S3 & 0.720 & 0.684 & 0.448 & 4.987 & 37.768 \\ \midrule
S4 & 0.635 & 0.576 & 0.393 & 9.221 & 37.909 \\ \midrule
Leaves & 0.278 & 0.211 & 0.016 & 24.236 & 94.235 \\ \midrule
letter1 & 0.264 & 0.268 & 0.408 & -1.756 & -54.783 \\ \midrule
letter2 & 0.164 & 0.166 & 0.204 & -1.458 & -24.324 \\ \midrule
letter3 & 0.196 & 0.193 & 0.254 & 1.613 & -29.403 \\ \midrule
letter4 & 0.162 & 0.153 & 0.135 & 5.476 & 16.773 \\ \midrule
M1 & 0.756 & 0.640 & 0.519 & 15.298 & 31.355 \\ \midrule
M2 & 0.483 & 0.393 & 0.190 & 18.606 & 60.545 \\ \midrule
M3 & 0.353 & 0.291 & 0.137 & 17.603 & 61.162 \\ \midrule
M4 & 0.246 & 0.226 & 0.070 & 7.814 & 71.675 \\ \midrule
\multicolumn{4}{|l|}{Avg-all Datasets} & 7.954 & 25.819 \\ \bottomrule
\end{tabular}}
%\end{table}


==> unified_algorithm.tex <==
\section{Framework to Organize Several K-Medoid Algorithms}
\label{section_framework_to_organize_several_k_medoid_algorithms}

With a small generalization to the previous setting, we get a framework that loosely contains
many K-medoids algorithms.
Consider two, possibly independent, samples from $\underlyingSpace$: $\{x_i\}$ $i = [1,m]$ 
and $\{y_j\}$ $j = [1,n]$. 
$\kTupleSample$ is constructed from $\{x_i\}$ and 
$\{y_j\}$ is used for estimating eccentricities.

Many K-medoid algorithms can be conceptually viewed as the interplay of two 
optimization avenues: 
(i) better sampling of candidate medoids $\kTupleSample$, possibly by varying $m$
(ii) better estimation of eccentricity of sampled candidates,
    possibly by varying $n$.
We turn this into a framework: GPAM (Generalized PAM) is defined to take in 
$\{x_i\}$, $\{y_j\}$
with arbitrary (in)dependence (listings \ref{algorithm_GPAM_INNER}, \ref{algorithm_GPAM_OUTER}).
GPAM is parametrized by the input $\{x_i\}$, $\{y_j\}$,
this is concisely denoted as GPAM(m, n).
The initial choice of $\candidateMedoid$ can be done by any standard intialization routine.
GPAM\_INNER is calculating the sample medoid of the k-points constructed
by swapping the $k$ slots of $\candidateMedoid$ with $m$ points of $\{x_i\}$
and $\errFour$ is the true error of GPAM\_INNER.

\begin{algorithm}
\caption{GPAM\_INNER}
\label{algorithm_GPAM_INNER}
\begin{algorithmic}[1]
\REQUIRE Candidate k-medoid $\candidateMedoid$, $\EccHat(\candidateMedoid)$;
    samples $\{x_i\}, \{y_{ilj}\}$, $i = [1,m]$ $l = [1,k], j = [1,n]$
\FOR{$i = 1$ to $m$}
    \FOR{$l = 1$ to $k$}
    \STATE $\candidateMedoidSwap \leftarrow \candidateMedoid$;
        $\candidateMedoidSwap[l] \leftarrow x_i$
        \quad \COMMENT{$\kTupleSample$ construction by swapping elements of $\candidateMedoid$}
    \STATE $\EccHat(\candidateMedoidSwap) \leftarrow \frac{1}{n} \sum_{j = 1}^n d(y_{ilj}, \candidateMedoidSwap)$
    \IF{$\EccHat(\candidateMedoidSwap) < \EccHat(\candidateMedoid)$}
        \STATE $\candidateMedoid \leftarrow \candidateMedoidSwap$; $\EccHat(\candidateMedoid) \leftarrow \EccHat(\candidateMedoidSwap)$
    \ENDIF
    \ENDFOR
\ENDFOR
\RETURN $\candidateMedoid, \EccHat(\candidateMedoid)$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{GPAM\_OUTER}
\label{algorithm_GPAM_OUTER}
\begin{algorithmic}[1]
\REQUIRE Candidate k-medoid $\candidateMedoid \in \kTupleSpace$, $\EccHat(\candidateMedoid)$;
    samples $\{x_i\} \subset \underlyingSpace$, $i = [1,m]$;
    samples $\{y_{ilj}\} \subset \underlyingSpace$, $l = [1,k], j = [1,n]$

    \STATE $\candidateMedoidUpdated, \EccHat(\candidateMedoidUpdated) \leftarrow 
    \text{GPAM\_INNER}(\candidateMedoid, \EccHat(\candidateMedoid), \{x_i\}, \{y_{ilj}\})$
    \IF{$\EccHat(\candidateMedoid) - \EccHat(\candidateMedoidUpdated) > \text{TOL}$}
        \STATE $\candidateMedoid \leftarrow \candidateMedoidUpdated$; $\EccHat(\candidateMedoid) \leftarrow \EccHat(\candidateMedoidUpdated)$
        \STATE \textbf{repeat} from 1
    \ENDIF

\RETURN $\candidateMedoid, \EccHat(\candidateMedoid)$
\end{algorithmic}
\end{algorithm}

The widespread applicability of $\errFour$ will now become apparent,
since a number of K-medoid algorithms formally or loosely fit into the GPAM framework.
If $\{y_j\} = \{x_i\}$, ($n = m$)
and set $y_{ilj} = y_j$ for all $i,l$ (i.e repeat the $y_j$), then
PAM = CLARA = GPAM(m, m).
CLARA  \cite{kaufman2008clustering} typically sets $m$ much smaller than PAM \cite{kaufman1990partitioning}, 
and does multiple reruns.
If $\{x_i\}$ is a randomly permuted subset of $\{y_j\}$, ($m << n$),
then CLARANS \cite{ng2002clarans} is GPAM(m, n) with the modification that on a successful swap 
(GPAM\_INNER line 6), GPAM\_INNER exits immediately.
When $k = 1$ and $\{y_j\}$ is sampled with replacement from $\{x_i\}$, ($m >> n$),
RAND \cite{eppstein2001fast} is GPAM\_INNER(m, n). 
TOPRANK \cite{okamoto2008ranking} is several repeated applications of RAND, by taking the best medoids
from the previous run and then increasing $n$,
followed by a final exact calculation. Hence
TOPRANK is intimately connected to GPAM\_INNER(m, n).
Understanding the dynamics of GPAM for different regimes of $m$ and $n$,
will give a broad understanding of this algorithmic landscape. 
We provide a substantial characterization of GPAM by analyzing GPAM\_INNER in section
\ref{section_kmedoids_theory_results}.

While other algorithms do not use the sample medoid as the estimator,
they follow the general idea of sampling either $\{y_j\}$ or $\{x_i\}$
to identify better medoids. The 1-medoid algorithms trimed
(triangle inequality based eccentricity bounding) \cite{newling2016sub} and 
meddit (multi-armed bandits based sample medoid estimation) \cite{bagaria2017medoids} work in the 
regime $m >> n$. PAMAE (hybrid of CLARA and 'K-means' style approach) \cite{song2017pamae} 
works in the $m = n$ regime.

